AMUSED: A Multi-Stream Vector Representation Method for Use in Natural Dialogue

The problem of building a coherent and non-monotonous conversational agent with proper discourse and coverage is still an area of open research. Current architectures only take care of semantic and contextual information for a given query and fail to completely account for syntactic and external knowledge which are crucial for generating responses in a chit-chat system. To overcome this problem, we propose an end to end multi-stream deep learning architecture which learns unified embeddings for query-response pairs by leveraging contextual information from memory networks and syntactic information by incorporating Graph Convolution Networks (GCN) over their dependency parse. A stream of this network also utilizes transfer learning by pre-training a bidirectional transformer to extract semantic representation for each input sentence and incorporates external knowledge through the the neighborhood of the entities from a Knowledge Base (KB). We benchmark these embeddings on next sentence prediction task and significantly improve upon the existing techniques. Furthermore, we use AMUSED to represent query and responses along with its context to develop a retrieval based conversational agent which has been validated by expert linguists to have comprehensive engagement with humans.

==> sections/overview.tex <==
%\section{Task Definition}
%The task of relation extraction in multi-instance setting involves a list of bags $\{B_1, B_2, ... , B_n\}$ for training, where each bag $B_i$ is labeled with a triplet from KB and contains multiple sentences (instances) $\{s_i^1, s_i^2, ... s_i^m\}$. The objective is to predict the relation in unseen bags between the given entity pair.

\section{\method{} Overview}
\label{sec:overview}

\method{} consists of three main components. We briefly present them below and the subsequent sections will cover them in greater depth. \method{}'s overall architecture is shown in \reffig{fig:model_overview}.

%A given sentence $x$ when passed through the network is encoded into a representation $\phi(x)$ which is the concatenation of vectors $\phi_{gcn}(x)$ and $\phi_{trans}(x)$ generated from the streams of (GRU,GCN) and transformer lookup respectively.  It can be represented by:
%\[ \phi(x) =[\phi_{gcn}(x), \phi_{trans}(x)] \]
%The representation $\phi(q)$ for a qeury q along with its context list $(l)$ is passed further through the memory network to get a new representation $\phi^+(q)$. The vectors for answer$(a)$ and negative$(n)$ are not required to be passed through the memory network.

%The final representations for a triplet is hence defined by $(\phi^+(q), \phi(a), \phi(n))$ and is used to optimize the network using triplet loss.

%The subsequent sections will cover individual parts of AMUSED in greater depth:

\subsection{Syntactic Module}
%We propose a multi-stream end to end architecture
%(AMUSED) for a retrieval based chit-chat system that is
%trained on triplet loss to generate information rich embeddings
%for a given query. The architecture consists of a 2 -stream
%network where the first stream encodes a given query by
%passing through a series of Bi-directional GRU and GCN
%layers and the second stream uses sentence embeddings
%generated using BERT. The second stream has a transfer
%learning framework where semantic representation for each
%query is extracted using a BERT model[2] which has been pre
%trained on next dialogue prediction task. Both the embeddings
%are further concatenated and passed through a memory
%network to incorporate contextual information for each
%conversation. The network uses triplets(query, response,
%negatives) as input and is optimized by triplet loss.
%For a given user query, responses are generated by first
%subsampling a set of responses having overlapping key words
%and then performing cosine similarity to select the most
%probable response.
The syntactic module of \method{} consists of a Bi-\lstm{} over the word embeddings of the input tokens. A syntactic GCN is employed over the dependency parse of the tokens to capture long-range syntactic information. The Bi-\lstm{} embedding is then concatenated with the GCN embedding to get a syntax-enriched embedding for the sentence. More details in \refsec{sec:syntactic_module_details}.

\subsection{Knowledge Module}
In this part, the input sentence is passed to a BERT model which is pre-trained on the task of next dialogue prediction, to obtain a sentence embedding from BERT. This embedding is augmented with the average of the embeddings of nodes which are at one-hop distance in the neighborhood of entity-linked tokens of the input. The details about the linking and k-hop expansion are given in \refsec{sec:knowledge_module_details}.

\subsection{Memory Module}
This module is used to make our network context-aware. Here, a context is formed by using BERT embeddings of the previous queries and responses, which are then passed through a memory network to effectively capture the conversation context. During training time, only the query embedding from previous steps is passed to this module as described in \refsec{sec:memory_module_details}.

